Gujarati-English Code-Switching Speech Recognition using ensemble prediction of spoken language

An important and difficult task in code-switched speech recognition is to recognize the language, as lots of words in two languages can sound similar, especially in some accents. We focus on improving performance of end-to-end Automatic Speech Recognition models by conditioning transformer layers on language ID of words and character in the output in an per layer supervised manner. To this end, we propose two methods of introducing language specific parameters and explainability in the multi-head attention mechanism, and implement a Temporal Loss that helps maintain continuity in input alignment. Despite being unable to reduce WER significantly, our method shows promise in predicting the correct language from just spoken data. We introduce regularization in the language prediction by dropping LID in the sequence, which helps align long repeated output sequences.

==> Declaration.tex <==
\clearpage
\thispagestyle{empty}

\begin{center}
\Large  {\bf Declaration }
\end{center}
\vspace{-6in}
I declare that this written submission represents my ideas in my own words and where others ideas or words have been included, I have adequately cited and referenced the original sources. I also declare that I have adhered to all principles of academic honesty and integrity and have not misrepresented or fabricated or falsified any idea/data/fact/source in my submission. I understand that any violation of the above will be cause for disciplinary action by the Institute and can also evoke penal action from the sources which have thus not been properly cited or from whom proper permission has not been taken when needed.
\vspace{0.5in}

%\begin{flushleft}
%Date:
%\end{flushleft}
%\begin{flushright}
%Surendar M\\
%(Roll. No. 114310007)
%\end{flushright}


%
 \begin{table}[h]
 \begin{flushleft}

\vspace{-3.2in} 
 \begin{tabular}{ccccc}
 % %\hline 	\rule[5ex]{0pt}{-10ex} &&(Signature) (Date) && \\ 
 \rule[5ex]{0pt}{-10ex}&& Date: && \\ 
 \end{tabular}
\end{flushleft}

\vspace{-0.5in} 
\begin{flushright}
 \begin{tabular}{ccccc}
 % %\hline 	\rule[5ex]{0pt}{-10ex} &&(Signature) (Date) && \\ 
 
 \hline 	\rule[5ex]{0pt}{-10ex}&& Student Name&& \\ 
 \rule[5ex]{0pt}{-10ex}&& Roll No. 19XXXX&& \\ \\
 \end{tabular}
\end{flushright}
\end{table}

\pagebreak

==> abbreviations.tex <==
\chapter*{List of Abbreviations}
\label{ch:ListOfAbr}
\addcontentsline{toc}{chapter}{\nameref{ch:ListOfAbr}}

% \makeatletter
\newcommand{\tocfill}{\cleaders\hbox{}\hfill}
%\newcommand{\tocfill}{\cleaders\hbox{$\m@th \mkern\@dotsep mu . \mkern\@dotsep mu$}\hfill}
% \makeatother
\newcommand{\abbrlabel}[1]{\makebox[3cm][l]{\textbf{#1}\ \tocfill}}
\newenvironment{abbreviations}{\begin{list}{}{\renewcommand{\makelabel}{\abbrlabel}
                                              \setlength{\itemsep}{0pt}}}{\end{list}}
%\begin{abbreviations}[labelsep=1em,font=\bfseries]
\begin{abbreviations}
\item[STC] 	Seamless Temporal Classification
% \item[API] Application Programming Interface
% \item[BSC]	Backscattering Coefficient
% \item[SAR]  Synthetic Aperture Radar  
% \item[CTD]	Coherent Target Decomposition
\end{abbreviations}


==> approval.tex <==
\chapter*{}
\thispagestyle{empty}
\vspace{-1in}
\begin{center}
{\Large  {\bf Thesis Approval}}
\end{center}
\vspace*{0.1in} \noindent This thesis entitled {\large \bf Thesis title} by {\bf \large
Student Name} is approved for the degree of  {\large \bf Doctor of Philosophy}.\\\\
\hspace*{4 in} Examiners:\\\\
\hspace*{3.5 in} \ldots\ldots \ldots \ldots \ldots \ldots\ldots
\ldots \ldots \ldots\ldots\\\\
\hspace*{3.5 in} \ldots\ldots \ldots \ldots \ldots \ldots\ldots
\ldots \ldots \ldots\ldots\\\\
\hspace*{3.5 in} \ldots\ldots \ldots \ldots \ldots \ldots\ldots
\ldots \ldots \ldots\ldots\\\\
  \hspace*{3.5in} \ldots\ldots \ldots \ldots \ldots \ldots\ldots
\ldots \ldots \ldots\ldots\\\\
 Supervisor:\hspace*{3.5 in}  Chairperson:\\\\\\
\ldots\ldots \ldots \ldots \ldots \ldots\ldots
\ldots \ldots \ldots\ldots
\hspace*{1.0 in} \ldots\ldots \ldots \ldots \ldots \ldots\ldots
\ldots \ldots \ldots\ldots\\\\\\
%  \hspace*{4 in} Chairman:\\\\
% \hspace*{3.8 in} \ldots\ldots \ldots \ldots \ldots \ldots\ldots
% \ldots \ldots \ldots\ldots

\noindent
Date: \ldots\ldots \ldots \ldots\\\\
Place: \ldots\ldots \ldots \ldots
%\pagebreak \clearpage{\pagestyle{empty}\cleardoublepage}
% \clearpage{\pagestyle{empty}\cleardoublepage}

